Aligning Backchannel and Dialogue Context Representations via Contrastive LLM Fine-Tuning

Backchannels (e.g., `yeah', `mhm', and `right') are short, non-interruptive feedback signals whose lexical form and prosody jointly convey pragmatic meaning. While prior computational research has largely focused on predicting backchannel timing, the relationship between lexico-prosodic form and meaning remains underexplored. We propose a two-stage framework: first, fine-tuning large language models on dialogue transcripts to derive rich contextual representations; and second, learning a joint embedding space for dialogue contexts and backchannel realizations. We evaluate alignment with human perception via triadic similarity judgments (prosodic and cross-lexical) and a context-backchannel suitability task. Our results demonstrate that the learned projections substantially improve context-backchannel retrieval compared to previous methods. In addition, they reveal that backchannel form is highly sensitive to extended conversational context and that the learned embeddings align more closely with human judgments than raw WavLM features.

==> diagram.tex <==
\begin{tikzpicture}[
    node distance=1.5cm and 2cm,
    % Define standard styles for consistency
    box/.style={rectangle, draw=black, thick, minimum width=3cm, minimum height=1cm, align=center, rounded corners, fill=white},
    input/.style={trapezium, draw=black, thick, trapezium left angle=70, trapezium right angle=110, minimum width=2.5cm, align=center, fill=gray!10},
    embedding/.style={rectangle, draw=black!60, fill=blue!5, thick, minimum width=0.8cm, minimum height=2cm, align=center},
    loss/.style={circle, draw=red, thick, fill=red!10, minimum size=2.5cm, align=center, font=\bfseries},
    concat/.style={rectangle, draw=black, thick, fill=yellow!20, minimum width=5cm, minimum height=0.8cm, rounded corners, align=center, font=\bfseries},
    arrow/.style={-Latex, thick}
]

% =====================
% LEFT TOWER: Multimodal Context
% =====================

% --- Inputs (Side by Side) ---
\node[input] (text_in) {Dialogue Transcript\\(Text History)};
\node[input, right=1cm of text_in] (ctx_audio_in) {Last 1s Context\\(Audio Waveform)};

% --- Encoders (Side by Side below inputs) ---
\node[box, below=0.8cm of text_in, fill=blue!10] (llm) {\textbf{LLM Encoder}\\(Text Branch)};
\node[box, below=0.8cm of ctx_audio_in, fill=orange!10] (wavlm_ctx) {\textbf{WavLM Encoder}\\(Context Audio)};

% --- Concatenation Step ---
% Calculate center point below the two encoders
\coordinate (mid_encoders) at ($(llm.south)!0.5!(wavlm_ctx.south)$);
\node[concat, below=0.8cm of mid_encoders] (concat_node) {Concatenate [LLM Representation || WavLM Representation]};

% --- Projection & Embedding ---
\node[box, below=0.8cm of concat_node] (proj_ctx) {Projection Layer\\(Map to Joint Space)};
\node[embedding, below=0.8cm of proj_ctx, label=left:Multimodal Context Emb $z_{mc}$] (emb_ctx) {};


% =====================
% RIGHT TOWER: Feedback Audio
% =====================

% Positioning relative to the far right of the context tower to ensure spacing
\node[input, right=4cm of ctx_audio_in] (fb_audio_in) {Backchannel\\(Feedback Audio)};
% Align WavLM feedback encoder horizontally with WavLM context encoder
\node[box, below=0.8cm of fb_audio_in, fill=orange!10] (wavlm_fb) at (fb_audio_in |- wavlm_ctx) {\textbf{WavLM Encoder}\\(Feedback Audio)};
% Align projection horizontally with context projection
\node[box, below=0.8cm of wavlm_fb] (proj_fb) at (wavlm_fb |- proj_ctx) {Projection Layer\\(Map to Joint Space)};
\node[embedding, below=0.8cm of proj_fb, label=right:Feedback Emb $z_{fb}$] (emb_fb) {};


% =====================
% LOSS FUNCTION
% =====================
\coordinate (midpoint_embs) at ($(emb_ctx)!0.5!(emb_fb)$);
\node[loss, below=1cm of midpoint_embs] (loss_node) {Contrastive\\Loss\\($\mathcal{L}_{NCE}$)};


% =====================
% CONNECTIONS (Arrows)
% =====================

% Left Tower Flow
\draw[arrow] (text_in) -- (llm);
\draw[arrow] (ctx_audio_in) -- (wavlm_ctx);
\draw[arrow] (llm.south) -- (concat_node.north -| llm.south); % Connect down to concat box
\draw[arrow] (wavlm_ctx.south) -- (concat_node.north -| wavlm_ctx.south); % Connect down to concat box
\draw[arrow] (concat_node) -- (proj_ctx);
\draw[arrow] (proj_ctx) -- (emb_ctx);

% Right Tower Flow
\draw[arrow] (fb_audio_in) -- (wavlm_fb);
\draw[arrow] (wavlm_fb) -- (proj_fb);
\draw[arrow] (proj_fb) -- (emb_fb);

% Flow to Loss
\draw[arrow, dashed, very thick, blue!50!black] (emb_ctx.south) -- (loss_node.north west) node[midway, left, font=\footnotesize] {Align};
\draw[arrow, dashed, very thick, orange!50!black] (emb_fb.south) -- (loss_node.north east) node[midway, right, font=\footnotesize] {Align};


% =====================
% BACKGROUND GROUPING
% =====================
\begin{pgfonlayer}{background}
    % Multimodal Context Group
    \node[fit=(text_in)(ctx_audio_in)(concat_node)(emb_ctx), draw=blue!30, dashed, inner sep=0.6cm, rounded corners, fill=blue!2, label={[blue!60]above:\textbf{Multimodal Context Branch (Phase 2)}}] {};
    % Feedback Group
    \node[fit=(fb_audio_in)(wavlm_fb)(emb_fb), draw=orange!30, dashed, inner sep=0.6cm, rounded corners, fill=orange!2, label={[orange!60]above:\textbf{Feedback Branch}}] {};
\end{pgfonlayer}

\end{tikzpicture}
